Voxel2Hemodynamics: An End-to-end Deep Learning Method for Predicting Coronary Artery Hemodynamics

Local hemodynamic forces play an important role in determining the functional significance of coronary arterial stenosis and understanding the mechanism of coronary disease progression. Computational fluid dynamics (CFD) have been widely performed to simulate hemodynamics non-invasively from coronary computed tomography angiography (CCTA) images. However, accurate computational analysis is still limited by the complex construction of patient-specific modeling and time-consuming computation. In this work, we proposed an end-to-end deep learning framework, which could predict the coronary artery hemodynamics from CCTA images. The model was trained on the hemodynamic data obtained from 3D simulations of synthetic and real datasets. Extensive experiments demonstrated that the predicted hemdynamic distributions by our method agreed well with the CFD-derived results. Quantitatively, the proposed method has the capability of predicting the fractional flow reserve with an average error of 0.5\% and 2.5\% for the synthetic dataset and real dataset, respectively. Particularly, our method achieved much better accuracy for the real dataset compared to PointNet++ with the point cloud input. This study demonstrates the feasibility and great potential of our end-to-end deep learning method as a fast and accurate approach for hemodynamic analysis.

==> Parts/Reference.tex <==
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017

\end{thebibliography}

==> Parts/formula.tex <==
Unet
\begin{equation}
.\min _{\theta_U} \sum_{i=1}^N(L_{c e}\left(f_U\left(x_{U_i} ; \theta_U\right), y_{U_i}\right)+L_{\text {dice }} (f_U\left(x_{U_i} ; \theta_U\right), y_{U_i} ))
\end{equation}

MdNet
\begin{equation}
\min _{\theta_M} \sum_{i=1}^N L_{\text {mesh }}\left(f_M\left(x_{M i}, f_{U-D} ; \theta_M\right), y_{M_i}\right)
\end{equation}

PointNet
\begin{equation}
\min _{\theta P} \sum_{i=1}^N L_{\text {mse }}\left(f_P\left(x_{P_i}, f _{U-D}, h_t ; \theta_P\right), y_{P_i}\right)
\end{equation}



